Carbonyl4: A Sketch for Set-Increment Mixed Updates

In the realm of data stream processing, the advent of SET-INCREMENT Mixed (SIM) data streams necessitates algorithms that efficiently handle both SET and INCREMENT operations. We present Carbonyl4, an innovative algorithm designed specifically for SIM data streams, ensuring accuracy, unbiasedness, and adaptability. Carbonyl4 introduces two pioneering techniques: the Balance Bucket for refined variance optimization, and the Cascading Overflow for maintaining precision amidst overflow scenarios. Our experiments across four diverse datasets establish Carbonyl4's supremacy over existing algorithms, particularly in terms of accuracy for item-level information retrieval and adaptability to fluctuating memory requirements. The versatility of Carbonyl4 is further demonstrated through its dynamic memory shrinking capability, achieved via a re-sampling and a heuristic approach. The source codes of Carbonyl4 are available at GitHub.

==> note.tex <==
Title:
An Approximate Hash Table for Assignment-Increment Mixed Updates
An Approximate Hash Table for Set-Append Mixed Updates


Abstract:
extract item-level information?
Streaming key-value updates

Intro:


1.1 motivation
第一段：也许可以从sketch开始介绍。
sketch是一种能够维护per item信息的近似算法，在大量领域得到应用。相比于。。。的哈希表，sketch的优势在能使用压线性空间取得可控的精度和高速。此外sketch的大小可以自由配置，算法会自动在已分配的空间下做到尽可能好的精度。在高性能交换机、物联网、便携终端、传感器端侧等场景中，存储空间较少，且没必要提供100\%准确的测量结果，sketch成为更好的选择。

第二段：Limitations of sketches
但是sketch支持的数据流更新形式有限，和哈希表的核心功能差距在于其无法支持set操作。介绍两种更新并且定义。

第三段：applications
move "Sensor Data Collection" to the first application?

第四段。our goal
目前，因为sketch无法支持set，AIM的解决方案仅限于哈希表。我们的目标是设计一种支持AIM的sketch，也即是一种Approximate Hash Table。它将解决存储空间不足时精确哈希表不可用的问题，填补该场景下解决方案的空白，让上述三个和更多的应用受益。

参考表格：
 \begin{table}[h]
\centering
\begin{tabular}{|l|l|l|}
\hline
\textbf{}          & \textbf{Exact}                & \textbf{Approximate}        \\ \hline
\textbf{Increment-only} & Hash Tables                  & Sketches                    \\ 
\textbf{AIM}            & Hash Tables                   & Our work      \\ \hline
\end{tabular}
\caption{Your table caption here}
\label{your-label-here}
\end{table}


1.2 Limitations
第五段 Sketch为什么有问题
这里我们详细分析现有sketch为什么无法支持set。

1.3 our solution
第六段
不要分ideal和我们的方案了，直接说我们设计了一个什么东西取得了什么结果

第七段  （应该更详细地阐述为什么value大是一个问题，让人理解这个问题，再给方案，不然直接进入语境外行读不懂。）

在研究过程中，我们遇到了两个依次递进的挑战。
1、set可行性挑战。如何修改一个key的value使得整体算法功能不受破坏。比如，count sketch会通过key哈希选择的三个随机counter来给value一个无偏估计，如果我们直接把这三个counter修改为set的目标值，会导致其它使用这三个counter任意之一的key受到影响。对此我们进行了分析，阐明了可以set value的必要条件。

2、数据动态性挑战。传统以1为增量修改的append数据流只会缓慢地对数据结构里的元素value进行调整。而set操作可能会在一个操作里插入一个很大的value，这就需要数据结构具有非常好的动态性来容纳这些大value。对此，我们设计了。。。。。。





Section 2
介绍coco的merge的时候，说coco的关键技术是"unbiased merge"，但是这个merge针对“正数”，即increment only。

section3
开头介绍merge的时候，不要讲拓展coco的merge，而是扩展现有的unbiased merge。 可以增加一些rationale，section开头讲的还不够，一下从“how to use a single
Carbonyl4 bucket to handle Assignment-Increment mixed data
streams for unbiased and local optimal variance，”跳跃到"extend the MERGE" 有一点点突兀，可以加一两句话转折，介绍这个extend和AIM的关联，我们也希望支持append里的decrement

theorem1之前加一句：我们通过如下定理说明我们的merge cost是optimal的：



“For an incoming operation
⟨e′, “:=”, v′⟩, there are four possible cases as follows:” 这句话里没提到insertion，感觉提到这个词会好一点，不然句意有点含糊。

e'和section里对'的定义似乎不一致，也和e1 e2不一致，最好统一方便阅读。

\textit{“The Rationale of Carbonyl Bucket: In Cocosketch”  也许可以把Cocosketch 改成increment only solutions}

Theorem 2.的Q(e)这个符号最好能在Point query: 这段里就出现。

Assignment-Increment mixed data stream可以简化成AIM，觉得有点冗长。

感觉可以有更简短的一行的说法：“Proof. The detailed proofs of Theorem 2 and Theorem 3 are
shown in Section V-A.”




B. Carbonyl4 with Carbonyl Searching
要有过渡： 我们介绍了Carbonyl Bucket，但它的容量无法无限增加，否则将降低处理吞吐。因此我们进一步介绍完整的Carbonyl Sketch，它以Carbonyl Bucket为基本单元进行工作。

\textit{这里要不要写成两个子表的形式，保证h1 h2定位到的桶不是同一个？不然可能会有点小问题。}
“B1, · · · , Bn” 下标不对吧，应该是Bw？

Searching Stage 这里没有说明具体从哪个hashed bucket开始，如果是随机一个，就要明确说随机一个。
% Otherwise, we randomly select one of the two hashed buckets and use the following routine to perform a \textbf{Carbonyl Searching} to find a near-globally optimal selection for entries merging.


“ It is worth noting that if we find a bucket with
empty entry during the searching stage, then minglobal = 0,
and the kicking stage will also end at this bucket with an
% empty entry.”   在这个地方可以小discussion一下，说cuckoo有类似的操作，cuckoo hashing是要求minglobal=0才停止的一种特例吗？不知道这么讲对不对，好像也不一定对，因为cuckoo可以踢桶里任意一个。


Rationale有没有可能放到算法描述前面？算法细节比较多，如果先说怎么做，再说为什么，感觉对于外行来说会很难读，因为算法细节太复杂了，读的时候就得伴随思考为什么，不然很难直接记住细节。如果有个rationale的指引会比较好，即使rationale不好直接看懂，对读算法和example有帮助就好。

Theorem 4之前可以加一点自适应停止的discussion insight



section 5

可以简单写一两句为什么需要FLEXIBILITY、expand-
ing and shrinking，比如subsection B里说到“as shrinking the
memory footprint of a Carbonyl4 often means an urgent need
to allocate memory for more important applications.”，最好在开头这里就有铺垫，简单提到，而不是假设读者熟知FLEXIBILITY的意义。


A. Re-Build based Expanding and Shrinking


In-place Expanding: 这里没说insert的方法？如果insert过程中遇到illegal的怎么处理，如果引起illegal的爆炸，递归会不会出问题？


我感觉这一整个subsection A有点不太重要和啰嗦了，其实可以直接讲说我们把所有元素拿出来用目前的插入算法插入到一个新表里，几句话就得了，不用花这么多篇幅。


Heuristic也许放在Re-Sampling之前说更好，它更简明直接。

关于图表的建议：
Figure 1
不同case感觉可以用流程图来画（让人明确知道这是4个case），同时把左边的桶和右边的case分开。w.p.的另一侧可以写otherwise。容易让人误以为存在4~5个bucket。
如果想节约空间，可以把桶大小改成3或者2，4个元素有点偏多。

Figure 2
要直接地在图上标出B1.。。B8.  能不能不要写带小数点的例子？直接一位数可以吗？

Algorithm 1
建议把分号去掉，看着有点乱。注释稍微缩短一点，比如▷ calculate local optimal merge. 的merge可以去掉，find a new near-global optimal merge.可以改成 update global minimum
stop searching stage with a probability of pε.    stop w.p. pε.   

Algorithm 2:
类似Algorithm 1


Fig. 3: Re-Sampling Shrink. 增加文字描述。

Fig. 4: Heuristic Shrink. 增加文字描述。 放到figure 3之前更好。

Section 6
